Active Learning for Deep Object Detection

The great success that deep models have achieved in the past is mainly owed to large amounts of labeled training data. However, the acquisition of labeled data for new tasks aside from existing benchmarks is both challenging and costly. Active learning can make the process of labeling new data more efficient by selecting unlabeled samples which, when labeled, are expected to improve the model the most. In this paper, we combine a novel method of active learning for object detection with an incremental learning scheme to enable continuous exploration of new unlabeled datasets. We propose a set of uncertainty-based active learning metrics suitable for most object detectors. Furthermore, we present an approach to leverage class imbalances during sample selection. All methods are evaluated systematically in a continuous exploration context on the PASCAL VOC 2012 dataset.

==> include/autotable.tex <==
\begin{tabular}{c| c c c c }
Epoch &  14 & 14 & 59 & 59 \\
Metric & mAP & mF1 & mAP & mF1 \\
\hline
1avgproposalavg1vs210csv & 11.5 $\pm$ 2.1 & 27.1 $\pm$ 3.0 & 23.9 $\pm$ 1.2 & 46.8 $\pm$ 1.3\\
1avgproposalmax1vs210csv & 12.6 $\pm$ 2.0 & 28.8 $\pm$ 4.2 & 24.5 $\pm$ 0.7 & 47.5 $\pm$ 1.0\\
1avgproposalsum1vs210csv & 14.1 $\pm$ 1.3 & 32.3 $\pm$ 2.5 & 23.8 $\pm$ 1.2 & 46.4 $\pm$ 1.3\\
1avgrandom10csv & 12.0 $\pm$ 1.2 & 27.8 $\pm$ 2.9 & 23.4 $\pm$ 0.8 & 46.2 $\pm$ 1.3\\
1avgwholeimage1vs210csv & 14.0 $\pm$ 1.1 & 31.1 $\pm$ 2.1 & 23.7 $\pm$ 0.5 & 46.4 $\pm$ 0.5\\
1avgwholeimagediff10csv & 10.2 $\pm$ 1.6 & 23.9 $\pm$ 4.1 & 24.7 $\pm$ 1.7 & 47.7 $\pm$ 1.6\\
\end{tabular}


==> include/notations.tex <==
\usepackage{xspace}
\usepackage{xparse}
\usepackage{mathtools}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%DEEP-EMOC specific
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sqBrack}[1]{\left[#1\right]}
\newcommand{\rnBrack}[1]{\left(#1\right)}
\newcommand{\norm}[1]{\left|\left|#1\right|\right|}
%
\newcommand{\creg}{\mat{C}^{-1}_{reg}}
\newcommand{\sigmaf}{\sigma^2_f\rnBrack{\newx}}
%
\newcommand\sgdset{\mathcal{S}_{\text{sgd}}}
\newcommand\dataset{\mathcal{D}}
\newcommand\labelvector{\inputlabelvector}
\newcommand{\updateSet}{\ensuremath{\mathcal{S}_{\timestep}}}
%
\newcommand{\iterationSGD}{\ensuremath{t}}
\newcommand{\learningRate}{\ensuremath{\gamma}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % TEXT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\eg}{\emph{e.g.,}\xspace}
\newcommand{\ie}{\emph{i.e.,}\xspace}
\newcommand{\wrt}{\emph{w.r.t.}\xspace}
\newcommand{\etal}{\emph{et al.}\xspace}
%
\newcommand\myparagraph[1]{\vspace{3pt}\noindent\textbf{#1}\quad}
%
\newcommand{\ith}{\textsuperscript{th}\xspace}
%
\newcommand{\numberthis}{\addtocounter{equation}{1}\tag{\theequation}}

% minor tricks

\newcommand{\myspacex}{\phantom{x}}

%
\newcommand{\eqremark}[1]{\text{\textcolor{fsublue}{\textit{\scriptsize  \fbox{#1}}}}}

\newcommand{\mathtext}[1]{\ensuremath{\text{\normalfont #1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % BASIC MATH NOTATION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% matrix and vector notation
\renewcommand{\vec}[1]{\ensuremath{\mathbf{\boldsymbol{#1}}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{\boldsymbol{#1}}}}
%
\newcommand{\entryofvec}[2]{\ensuremath{#1\left(#2\right)}}
\newcommand{\dimofvec}[2]{\ensuremath{\entryofvec{#1}{#2}}}
%
\newcommand{\entryofmat}[3]{\ensuremath{#1\left(#2,#3\right)}}%{\ensuremath{#1_{#2,#3}}}

% vectors and matrices with 2 or 3 elements in row (and column)
\newcommand\mattwo[4]{\left[\begin{array}{cc} #1 & #2\\ #3 & #4 \end{array} \right]}
\newcommand\matthree[9]{\left[\begin{array}{ccc} #1 & #2 & #3\\ #4 & #5 & #6\\ #7 & #8 & #9 \end{array} \right]}
\newcommand\vectwo[2]{\left[\begin{array}{c} #1 \\ #2 \end{array} \right]}
\newcommand\vecthree[3]{\left[\begin{array}{c} #1 \\ #2 \\ #3 \end{array} \right]}

\newcommand{\diag}{\ensuremath{\text{diag}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % some standard vector spaces
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\numbersetpos}[1]{#1_{+}}
\newcommand{\numbersetnotneg}[1]{#1_{*}}

\newcommand{\N}{\mathbb{N}}
\newcommand{\Npos}{\numbersetpos{\N}}
\newcommand{\Nnotneg}{\numbersetnotneg{\N}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\Rpos}{\numbersetpos{\R}}
\newcommand{\Rnotneg}{\numbersetnotneg{\R}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % data and features space
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% feature space
%
\newcommand{\inputspace}{\ensuremath{\Omega}}
\newcommand{\dimension}{D}
%
\newcommand{\inputsingle}{\ensuremath{\vec{x}}}
\newcommand{\inputsingledim}{\ensuremath{x}}%make sure that this is the same as above just without vec

%
%labels
%
\newcommand{\labelspace}{\ensuremath{\mathcal{Y}}}
%
\newcommand{\labelsymbol}{y}
\newcommand{\labelsingle}{\labelsymbol}

\newcommand{\inputlabelvector}{\vec{\labelsymbol}}
\newcommand{\inputlabelset}{\mathrm{\labelsymbol}}

% data given
%
\newcommand{\noe}{\ensuremath{N}}
\newcommand{\numberOfExamples}{\noe}
%
\newcommand{\numberOfClasses}{\ensuremath{K}}
\newcommand{\noc}{\numberOfClasses}
\newcommand{\classRunning}{k}

\newcommand{\datasetLabeled}{\ensuremath{\mathfrak{L}}}
\newcommand{\datasetTest}{\ensuremath{\mathfrak{T}}}

\newcommand{\inputvectorsymbol}{X}
\newcommand{\inputdatamatrix}{\mat{\inputvectorsymbol}}
\newcommand{\inputvectorset}{\mathcal{\inputvectorsymbol}}
%

\newcommand{\inputnew}{\ensuremath{\inputsingle_*}}
\newcommand{\labelnew}{\ensuremath{\labelsingle_*}}

\newcommand{\numPixels}{\ensuremath{n_{px}}}
\newcommand{\powerset}{\mathfrak{P}}



%---------------------------------------
% % norms, set sizes
%---------------------------------------
\newcommand{\vectornorm}[1]{\left|\left|#1\right|\right|}
\newcommand{\setnorm}[1]{\left|#1\right|}
\newcommand{\matrixnorm}[1]{\left|#1\right|}
% \newcommand{\abs}[1]{\operatorname{abs}\left(#1\right)}
\newcommand{\abs}[1]{\left|#1\right|} %FIXME check that this version is fine everywhere
\newcommand{\frobnorm}[1]{\ensuremath{\matrixnorm{#1}_F}}
\newcommand{\infnorm}[1]{\ensuremath{\vectornorm{#1}_{\infty}}}


%---------------------------------------
% % differential symbol for integrals
%---------------------------------------
\newcommand{\diffd}{\operatorname{d}\!}
% \newcommand{\derivd}{\partial}


%---------------------------------------
% % further operators
%---------------------------------------

\newcommand{\innerproduct}[2]{\ensuremath{\langle#1,#2\rangle}}

\newcommand{\distancefunction}{\operatorname{d}}
\newcommand{\distanceEuclidian}{\operatorname{d}_{L_2}}
\newcommand{\distanceManhattan}{\operatorname{d}_{L_1}}
\newcommand{\distancechisquare}{\operatorname{d}_{\chi^2}}

\newcommand{\prob}{\ensuremath{p\!}}
%
\newcommand{\given}{\,|\,}

% \newcommand{\argmax}{\text{\normalfont{argmax}}}
% \newcommand{\argmin}{\text{\normalfont{argmin}}}
% \newcommand{\maximize}{\text{\normalfont{maximize}}}
% \newcommand{\minimize}{\text{\normalfont{minimize}}}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\maximize}{maximize}
\DeclareMathOperator{\minimize}{minimize}

\newcommand{\expectation}{\ensuremath{\mathbb{E}}}
\newcommand{\expectationOver}[1]{\ensuremath{\expectation_{#1}}}


\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\newcommand{\logfrac}[1]{\ensuremath{\dfrac{\log #1}{#1}}}


%---------------------------------------
% % well-known functions
%---------------------------------------
\DeclareMathOperator\erf{\mbox{erf}}
\newcommand{\indicatorFunction}{\ensuremath{\boldsymbol{1}}}
%
\newcommand{\diracFct}{\ensuremath{\delta}}
\newcommand{\diracMeasure}[2]{\ensuremath{\delta_{#1}\left( #2 \right)}}
%
\newcommand{\kroneckerdelta}[2]{\ensuremath{\delta_{#1,#2}}}

\DeclareMathOperator{\sgn}{\operatorname{sgn}}

%---------------------------------------
% % asymptotic stuff
%---------------------------------------
\newcommand{\asympO}[1]{\mathcal{O}\left(#1\right)}


%---------------------------------------
% % matrix stuff
%--------------------------------------
%with serifes
\newcommand{\T}{\ensuremath{\mathrm{T}}}
%
\DeclareMathOperator{\rk}{\operatorname{rk}}
\DeclareMathOperator{\tr}{\operatorname{tr}}
\newcommand{\matinv}[1]{\ensuremath{#1^{-1}}}
\newcommand{\identityMatrix}[1]{\ensuremath{\mat{I}_{#1}}}
\newcommand{\unitvector}[1]{\ensuremath{\vec{e}_{#1}}}
%
\newcommand{\eigenvalue}{\ensuremath{\lambda}}
\newcommand{\eigmin}{\ensuremath{\eigenvalue_{\min}}}
\newcommand{\eigmax}{\ensuremath{\eigenvalue_{\max}}}
%
\newcommand{\diagtwo}[2]{\ensuremath{\begin{bmatrix} #1 & 0\\ 0 & #2 \end{bmatrix}}}

%---------------------------------------
% % learning theory
%---------------------------------------
%
% model and modelspace / hypothesis, hypothesisspace
%
\newcommand{\hypothesisspace}{\ensuremath{\mathbb{H}}}
\newcommand{\hypothesis}{\ensuremath{h}}
%
\newcommand{\groundTruthFunction}{\ensuremath{g}}
\newcommand{\hypothesisOpt}{\ensuremath{\hypothesis_*}}
\newcommand{\model}{\ensuremath{\hat{\hypothesis}}}
\newcommand{\modelfunction}{\ensuremath{f}}% intermediate function, sometimes also latent %FIXME needs to be included in notation overview


\newcommand{\loss}{\ensuremath{\mathcal{L}}}
\newcommand{\learningObjective}{\ensuremath{\bar{\loss}}}%this is the overall training data loss + some additional stuff, e.g. for regularization
%
\newcommand{\zeroonelosstext}{$0/1$-loss\xspace}
\newcommand{\zerooneloss}{\loss_{0/1}}
%
\newcommand{\lonelosstext}{$L_1$-loss\xspace}
\newcommand{\loneloss}{\loss_{L_1}}
%
\newcommand{\ltwolosstext}{$L_2$-loss\xspace}
\newcommand{\ltwoloss}{\loss_{L_2}}
%
\newcommand{\loglosstext}{log-loss\xspace}
\newcommand{\logloss}{\loss_{\operatorname{log}}}

\newcommand{\hingeloss}{\loss_{H}}
\newcommand{\infinityloss}{\loss_{\infty}}


%
\newcommand{\modelfamily}{\ensuremath{\mathbb{F}}}

%
%
\newcommand{\risk}{\ensuremath{\mathcal{R}}}
\newcommand{\riskEmpirical}{\ensuremath{\risk_{\mathtext{emp}}}}
\newcommand{\riskRegularized}{\ensuremath{\risk_{\mathtext{reg}}}}
%
\newcommand{\riskEstimatedEmpirical}{\risk_{\expectation}}


%
\newcommand{\complexityPenalty}{\ensuremath{\mathcal{C}}}
\newcommand{\regularizationfunction}{\ensuremath{\omega}}
\newcommand{\shattercoefficient}{\ensuremath{N_{\mathtext{vc}}}}
\newcommand{\tradeoffRiskComplexity}{\ensuremath{\nu}}%lambda}

\newcommand{\errorlearning}{\ensuremath{\epsilon}}
\newcommand{\errorlearningprob}{\ensuremath{\prob_{\ \epsilon}}}


%---------------------------------------
% % simple distributrions
%---------------------------------------

\newcommand{\parameters}{\ensuremath{\vec{\theta}}}
\newcommand{\parameterspace}{\ensuremath{\Theta}}
\newcommand{\parametersOpt}{\ensuremath{\parameters_{*}}}
\newcommand{\parametersOptML}{\ensuremath{\parametersOpt^{\mathtext{ML}}}}
\newcommand{\parametersOptMAP}{\ensuremath{\parametersOpt^{\mathtext{MAP}}}}


\newcommand{\mean}{\mu}
\newcommand{\variance}{\sigma^2}

% normal distribution
\newcommand{\meanVec}{\vec{\mean}}
\newcommand{\covMat}{\mat{\Sigma}}
\newcommand{\normaldistributionsign}{\mathcal{N}}
\newcommand{\gaussdist}[3]{\ensuremath{\normaldistributionsign\left(#1 \given #2, #3\right)}}


%---------------------------------------
% % KNN
%---------------------------------------
\newcommand{\knn}{K}
\newcommand{\knnSet}{\mathcal{S}_{\knn}}

%---------------------------------------
% % LDA
%---------------------------------------
\newcommand{\weightVec}{\ensuremath{\vec{w}}} % weight vector
%
\newcommand{\ldaNeg}{{\vec{\mu}_{-1}}}
\newcommand{\ldaPos}{{\vec{\mu}_{1}}}
\newcommand{\ldaCov}{\covMat_0}
\newcommand{\ldaweight}{\weightVec_{\text{\normalfont{LDA}}}}




%---------------------------------------
% % SVM stuff
%---------------------------------------
\newcommand{\setofpoints}{\mathcal{S}}
\newcommand{\setofpointslinear}{\mathcal{S}_{\weightVec,\svmoffset}}
\newcommand{\distancefunctionpointtoset}{\distancefunction_{\bot}}

\newcommand{\svmoffset}{b}

\newcommand{\hypothesislinear}{\modelfunction_{\weightVec,\svmoffset}}
\DeclareMathOperator{\margin}{mg}
% \newcommand{\margin}{\text{\normalfont{mg}}}
\newcommand{\marginsymbol}{\Upsilon}
\newcommand{\svmCterm}{\ensuremath{C}}
\newcommand{\vcprob}{\ensuremath{\delta}}
\newcommand{\constant}{\ensuremath{c}}
\newcommand{\radius}{\ensuremath{R}}
\newcommand{\svmNumberOfMisclassification}{\ensuremath{k}}
\newcommand{\svmMarginPrecision}{\ensuremath{\rho}}
\newcommand{\svmslack}{\ensuremath{\xi}}
\newcommand{\svmslackvec}{\ensuremath{\vec{\xi}}}
\newcommand{\squashingfunction}{\ensuremath{s}}
%
%
\newcommand{\weightVecDual}{\ensuremath{\representersampleweightvec}} % weight vector in dual representation
\newcommand{\weightVecDualEntry}{\ensuremath{\representersampleweight}} % single entry of the vector in dual representation

% \newcommand{\representersampleweightvec}{\vec{\lagrangianmultiplier}}
% \newcommand{\representersampleweight}{\alpha}

%---------------------------------------
% optimization problems
%---------------------------------------

\newcommand{\optimizationProblem}[5]{
  \begin{equation}
      \label{#1}
      \begin{aligned}
	  & \underset{#3}{#2}              & & #4 \\
	  & \text{\normalfont{subject to}} & & #5\enspace.
      \end{aligned}
  \end{equation}
}

\newcommand{\optimizationProblemTwoConstraints}[6]{
  \begin{equation}
      \label{#1}
      \begin{aligned}
	  & \underset{#3}{#2}              & & #4 \\
	  & \text{\normalfont{subject to}} & & #5 \\
	  & \text{\normalfont{and}}        & & #6\enspace.
      \end{aligned}
  \end{equation}
}

\DeclareMathOperator{\lagrangian}{L}
\newcommand{\lagrangianmultipliervec}{\vec{\lagrangianmultiplier}}
\newcommand{\lagrangianmultiplier}{\lambda}
%
\newcommand{\representersampleweightvec}{\vec{\representersampleweight}}
\newcommand{\representersampleweight}{\alpha}

%---------------------------------------
% % kernel stuff
%---------------------------------------

\newcommand{\hyperparameter}{\eta}
\newcommand{\hyperparameters}{\ensuremath{\vec{\hyperparameter}}}

\newcommand{\featurespace}{\ensuremath{\mathcal{H}}}
\newcommand{\rkhs}{\ensuremath{\mathcal{H}}}

\newcommand{\featuretransform}{\Phi}
\newcommand{\featuretransformmat}{\mat{\Phi}}
\newcommand{\featuretransformvec}{\vec{\phi}}
\newcommand{\featuremap}{\featuretransform} % just a synonym
\newcommand{\featuretransformsecond}{\Psi}

\newcommand{\kernelfunction}{\kappa}
\newcommand{\kernellin}{\ensuremath{\kernelfunction_{\text{lin}}}}
\newcommand{\kernelpoly}{\kernelfunction_{\text{poly}}}
\newcommand{\kernelpolydegree}{p}
\newcommand{\kernelrbf}{\kernelfunction_{\text{RBF}}}
\newcommand{\kernelchisquare}{\kernelfunction_{\chi^2}}
\newcommand{\kernelHIK}{\ensuremath{\kernelfunction_{\text{HIK}}}}
\newcommand{\kernelGHIK}{\ensuremath{\kernelfunction_{\text{GHIK}}}}
\newcommand{\kernelHIKPOLY}{\ensuremath{\kernelfunction_{\text{HIK-POLY}}}}
\newcommand{\kernelHIKEXP}{\ensuremath{\kernelfunction_{\text{HIK-EXP}}}}
\newcommand{\kernelHIKARD}{\ensuremath{\kernelfunction_{\text{HIK-ARD}}}}

\newcommand{\sigmarbf}{\sigma}

%---------------------------------------
% % GP stuff
%---------------------------------------
\newcommand{\stochasticprocess}{\ensuremath{\mathtt{F}}}

\newcommand{\gpmeanfunction}{m}
\newcommand{\gpcovfunction}{\kernelfunction}
%
\newcommand{\kernelmatrixsymbol}{\ensuremath{K}}
\newcommand{\kernelmatrix}{\ensuremath{\mat{\kernelmatrixsymbol}}}
\newcommand{\kernelvectorsymbol}{\ensuremath{k}}
\newcommand{\kernelvector}{\ensuremath{\vec{\kernelvectorsymbol}_{*}}}
\newcommand{\kernelself}{\ensuremath{\kernelvectorsymbol_{**}}}
%

\newcommand{\latentfunction}{\modelfunction}
\newcommand{\latentfunctionvalue}{\stochasticprocess}
%
\newcommand{\latentfunctionvaluenew}{f_{*}}
%
\newcommand{\noiseprocess}{\varepsilon}%\eta}
\newcommand{\noise}{n}
\newcommand{\noisevariance}{\sigma_{\noise}^2}
\newcommand{\gpnoise}{\noisevariance} %just a synonym
\newcommand{\kernelmatrixreg}{\mat{\tilde{\kernelmatrixsymbol}}}


\newcommand{\covmatlinearregression}{\ensuremath{\mat{C}}}


\newcommand{\gpregmean}{\mean_{*}}%
\newcommand{\gpregvariance}{\variance_{*}}
\newcommand{\gpregstddev}{\sigma_*}
%
% gpregdev = gpnoise + gpregfvar

%
\newcommand{\gpregfvarnew}{\sigma_{\!f_*}^2} % variance of latent function value of test sample
\newcommand{\gpregfvar}{\sigma_{\!f}^2} % variance of latent function values

% cholesky decomposition
\newcommand{\choleskymatrixsymbol}{L}
\newcommand{\choleskymatrix}{\ensuremath{\mat{\choleskymatrixsymbol}}}
\newcommand{\choleskyentry}{\ensuremath{\ell}}


%---------------------------------------
% % IMAGES
%---------------------------------------
\newcommand{\image}{\ensuremath{\mathcal{I}}}



\newcommand{\localFeat}{\mathit{lf}}
\newcommand{\lfPos}{\vec{p}}
\newcommand{\lfDesc}{\vec{d}}
\newcommand{\lfNumFeat}{\mathcal{N}}
%---------------------------------------
% % codebook, quantization, ...
%---------------------------------------
\newcommand{\vectorquant}{\operatorname{vc}}
\newcommand{\codebook}{\mat{C}}
\newcommand{\prototype}{\vec{\mathfrak{p}}}
\newcommand{\lfNumPrototypes}{\mathfrak{K}}


%---------------------------------------
% % object detection
%---------------------------------------
\newcommand{\detector}{\ensuremath{\weightVec}}
\newcommand{\dpm}{\ensuremath{M_{DPM}}}
\newcommand{\numParts}{\ensuremath{n_p}}
\newcommand{\deformCost}{\ensuremath{\mathcal{L}_\mathcal{D}}}


%---------------------------------------
% % GPHIK
%---------------------------------------
\newcommand{\perm}{\ensuremath{\vec{\pi}}}
\DeclareMathOperator{\quant}{\ensuremath{\text{quant}}}
\DeclareMathOperator{\quantbinning}{\ensuremath{\text{binning}}}
\newcommand{\numbins}{\ensuremath{q}}
%  definitions for the proof in the appendix
\newcommand{\inputnewquant}{\ensuremath{\tilde{\inputsingle}_*}}
\newcommand{\maxquanterror}{\ensuremath{\varepsilon_{q}}}
\newcommand{\kernelvectorquant}{\ensuremath{\tilde{\vec{k}}_*}}
\newcommand{\gpregmeanquant}{\ensuremath{\tilde{\mean}_*}}
\newcommand{\deltaK}{\ensuremath{\triangle \kernelvector}}
%
\newcommand{\xtraindim}{\ensuremath{\dimofvec{\inputsingle_{i}}{d}}}
\newcommand{\xtestquantdim}{\ensuremath{\dimofvec{\inputnewquant}{d}}}
\newcommand{\xtestdim}{\ensuremath{\dimofvec{\inputnew}{d}}}
\newcommand{\deltaMin}{\ensuremath{\triangle{\min}_{*}^{i}\left(d\right)}}
% upper bound stuff
\DeclareMathOperator{\ub}{ub}
\newcommand{\tupper}{\ensuremath{\bar{t}}}
% for variance computations
\newcommand{\projKernelVector}{\ensuremath{\tilde{\vec{\kernelvectorsymbol}}_*}}
\newcommand{\projKernelInvMat}{\ensuremath{\vec{\nu}}}
\newcommand{\eigenvalueInvMat}{\ensuremath{\xi}}
\newcommand{\numEV}{\ensuremath{k}}
%  iteration counts
\newcommand{\iterationILS}{\ensuremath{T_1}}
\newcommand{\iterationDHS}{\ensuremath{T_2}}
\newcommand{\iterationArnoldi}{\ensuremath{T_3}}




%---------------------------------------
% % incremental learning stuff
%---------------------------------------
\newcommand{\numberofnewexamples}{\ensuremath{\noe_*}}
\newcommand{\none}{\ensuremath{\numberofnewexamples}}
%
\newcommand{\newx}{\ensuremath{\inputsingle'}}
\newcommand{\newy}{\ensuremath{\labelsingle'}}
%
\newcommand{\modelUpdated}{\ensuremath{\model'}}
\newcommand{\modelfunctionUpdated}{\ensuremath{\modelfunction'}}
\newcommand{\parametersUpdated}{\ensuremath{\parameters'}}
\newcommand{\kernelVectorUpdated}{\ensuremath{\kernelvector'}}
\newcommand{\weightVecDualUpdated}{\ensuremath{\weightVecDual'}}
%
\newcommand{\vecrankupdate}{\ensuremath{\vec{d}}}
\newcommand{\kernelmatrixnew}{\ensuremath{\mat{\kernelmatrixsymbol'}}}%{\ensuremath{\mat{\bar{\kernelmatrixsymbol}}}}
%
\newcommand{\choleskymatrixnew}{\ensuremath{\mat{\choleskymatrixsymbol'}}}%{\ensuremath{\mat{\bar{\choleskymatrixsymbol}}}}
\newcommand{\choleskyvectornew}{\ensuremath{\vec{\choleskyentry}_*}}
\newcommand{\choleskyentrynew}{\ensuremath{\choleskyentry_{**}}}
%
\newcommand{\weightvecdualnew}{\ensuremath{\vec{\representersampleweight'}}}%{\ensuremath{\vec{\bar{\representersampleweight}}}} % weight vector in dual representation
%
\newcommand{\timestep}{\ensuremath{t}}




%---------------------------------------
% % active learning stuff
%---------------------------------------
%
\newcommand{\activeLearning}{\ensuremath{\mathcal{AL}}}
%
\newcommand{\datasetUnlabeled}{\ensuremath{\mathfrak{U}}}
\newcommand{\datasetAll}{\ensuremath{\mathfrak{D}}}
%
\newcommand{\costFct}{\ensuremath{\operatorname{cost}}}
\newcommand{\costMax}{\ensuremath{\xi}}
\newcommand{\queryFct}{\ensuremath{\mathcal{Q}}}
%
\newcommand{\inputAL}{\ensuremath{\inputsingle'}}
\newcommand{\inputlabelAL}{\ensuremath{\labelsingle'}}
%
\newcommand{\modelAL}{\ensuremath{\modelfunction}}
\newcommand{\modelALOpt}{\ensuremath{\modelfunction_*}}
\newcommand{\modelALUpdated}{\ensuremath{\modelfunction'}}
%
\newcommand{\datasetSelectedSymbol}{\ensuremath{\mathfrak{S}}}
\newcommand{\datasetSelected}{\ensuremath{\datasetSelectedSymbol_*}}
\newcommand{\datasetSelectedPossibly}{\ensuremath{\datasetSelectedSymbol'}}
\newcommand{\inputALSelected}{\ensuremath{\inputsingle_*}}
%
\newcommand{\labelvecSelectedSymbol}{\ensuremath{\inputlabelvector}}
\newcommand{\labelvecSelected}{\ensuremath{\labelvecSelectedSymbol_*}}
\newcommand{\labelvecSelectedPossibly}{\ensuremath{\labelvecSelectedSymbol'}}
%
\newcommand{\changeSymbol}{\ensuremath{\Delta}}
\newcommand{\riskChange}{\ensuremath{\changeSymbol\risk}}
\newcommand{\empiricalRiskChange}{\ensuremath{\changeSymbol\riskEmpirical}}
\newcommand{\estimatedEmpiricalRiskChange}{\ensuremath{\changeSymbol\riskEstimatedEmpirical}}
\newcommand{\estimatedExpectedRiskChange}{\ensuremath{\changeSymbol\risk}}
%
\newcommand{\WeightVecDualChange}{\ensuremath{\changeSymbol \weightVecDual}}
%
\newcommand{\ModelChange}{\ensuremath{\changeSymbol \parameters}}
\newcommand{\lossOnModelRepresentations}{\ensuremath{\mathcal{L}_{\parameters}}} % {\ensuremath{\mathcal{L}_{\modelAL}}}
\newcommand{\lossOnModels}{\ensuremath{\mathcal{L}_{\modelAL}}} % {\ensuremath{\mathcal{L}_{\modelAL}}}
%
\newcommand{\ModelOutputChange}{\ensuremath{\changeSymbol \modelAL}}
%
\newcommand{\probLabeled}{\ensuremath{\boldsymbol{\prob}_{\ \datasetLabeled}}}
\newcommand{\probNew}{\ensuremath{\prob_{\ \inputAL}}}


%FIXME
%\newcommand\fvarInputAL{\sigma_{\!\model_*}^2} % variance of latent function value of test sample
\newcommand\fvarInputAL{\sigma_{\model}^2} % variance of latent function value of test sample



%
%FIXME generic symbols!
\newcommand{\ymulti}{\ensuremath{\bar{y}(\inputsingle)}}
\newcommand{\ymultiupdate}{\ensuremath{\bar{y}'(\inputsingle)}}
\newcommand{\ymultip}{\ensuremath{y}}
\newcommand{\rejectionClass}{\ensuremath{r}}
%---------------------------------------
% % density / unlabeled
%---------------------------------------

\newcommand{\pEmp}{\ensuremath{\prob_{\hspace{0.2em} \diracFct}}}
\newcommand{\pPDE}{\ensuremath{\prob_{\hspace{0.2em} \text{PDE}}}}



%---------------------------------------
% % patch discovery
%---------------------------------------
\newcommand{\patch}{\ensuremath{\vec{x}}}
\newcommand{\patchset}{\ensuremath{\mathcal{M}}}
\newcommand{\setAcceptable}{\ensuremath{\mathcal{A}}}
\newcommand{\numPatches}{\ensuremath{p}}
\newcommand{\numPatchesImg}{\ensuremath{p_{\image}}}
\newcommand{\numNewPatches}{\ensuremath{m}}
\newcommand{\numcells}{T}
\newcommand{\numchannels}{D_C}
\newcommand{\scores}{\ensuremath{\mathcal{S}}}
\newcommand{\combinationParameter}{\ensuremath{\lambda}}

%---------------------------------------
% % evaluation metrics
%---------------------------------------
\newcommand{\crossvalsplits}{\ensuremath{k}}
\newcommand{\accuracyEstimate}{\ensuremath{s}}
\newcommand{\ARR}{\ensuremath{\text{ARR}}}
\newcommand{\ORR}{\ensuremath{\text{ORR}}}
\newcommand{\confmat}{\ensuremath{M}}

%---------------------------------------
% % notations in experiments
%---------------------------------------

% GPHIK
\newcommand{\nneg}{\ensuremath{\ell}}

%active learning
\newcommand{\emocMC}{GP-EMOC$_{\text{MC}}$}
\newcommand{\emocPDE}{GP-EMOC$_{\text{PDE}}$}
\newcommand{\emocPDER}{GP-EMOC$_{\text{PDE+R}}$}

%---------------------------------------
% % deep learning stuff
%---------------------------------------
\newcommand{\numLayers}{\ensuremath{L}}

